Can Active Learning Experience Be Transferred?

Active learning is an important machine learning problem in reducing the human labeling effort. Current active learning strategies are designed from human knowledge, and are applied on each dataset in an immutable manner. In other words, experience about the usefulness of strategies cannot be updated and transferred to improve active learning on other datasets. This paper initiates a pioneering study on whether active learning experience can be transferred. We first propose a novel active learning model that linearly aggregates existing strategies. The linear weights can then be used to represent the active learning experience. We equip the model with the popular linear upper- confidence-bound (LinUCB) algorithm for contextual bandit to update the weights. Finally, we extend our model to transfer the experience across datasets with the technique of biased regularization. Empirical studies demonstrate that the learned experience not only is competitive with existing strategies on most single datasets, but also can be transferred across datasets to improve the performance on future learning tasks.

==> figure_tex/albl_talbl_mnist.tex <==
\begin{figure}[t]
\begin{center}
\centering
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/mnist_0vs1_albl_talbl_mnist.png}
                \caption{\textit{MNIST 0vs1}}
                \label{fig:mnist_albl_talbl_mnist}
        \end{subfigure}%
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/mnist_2vs3_albl_talbl_mnist.png}
    %            \caption{mnist 2vs3}
    %            \label{fig:mnist_albl_talbl_mnist}
    %    \end{subfigure}%
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/mnist_6vs7_albl_talbl_mnist.png}
    %            \caption{mnist 6vs7}
    %            \label{fig:mnist_albl_talbl_mnist}
    %    \end{subfigure}%
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/mnist_8vs9_albl_talbl_mnist.png}
                \caption{\textit{MNIST 8vs9}}
                \label{fig:mnist_albl_talbl_mnist}
        \end{subfigure}%

\end{center}
\caption{Test Accuracy of ALBL versus Transfer ALBL on \textit{MNIST}}
\label{fig:albl_talbl_mnist}
\end{figure}


==> figure_tex/albl_talbl_usps.tex <==
\begin{figure}[t]
\begin{center}
\centering
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/usps_0vs1_albl_talbl_usps.png}
                \caption{\textit{USPS 0vs1}}
                \label{fig:usps_0vs1_albl_talbl_usps}
        \end{subfigure}%
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/usps_4vs5_albl_talbl_usps.png}
    %            \caption{usps 4vs5}
    %            \label{fig:usps_4vs5_albl_talbl_usps}
    %    \end{subfigure}%
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/usps_6vs7_albl_talbl_usps.png}
    %            \caption{usps 6vs7}
    %            \label{fig:usps_6vs7_albl_talbl_usps}
    %    \end{subfigure}%
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/usps_8vs9_albl_talbl_usps.png}
                \caption{\textit{USPS 8vs9}}
                \label{fig:usps_8vs9_albl_talbl_usps}
        \end{subfigure}%

\end{center}
\caption{Test Accuracy of ALBL versus Transfer ALBL on \textit{USPS}}
\label{fig:albl_talbl_usps}
\end{figure}


==> figure_tex/lsa_tlsa_mnist.tex <==
\begin{figure}[t]
\begin{center}
\centering
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/mnist_0vs1_lsa_tlsa_mnist.png}
                \caption{\textit{MNIST 0vs1}}
                \label{fig:mnist_0vs1_lsa_tlsa_mnist}
        \end{subfigure}%
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/mnist_2vs3_lsa_tlsa_mnist.png}
    %            \caption{mnist 2vs3}
    %            \label{fig:mnist_2vs3_lsa_tlsa_mnist}
    %    \end{subfigure}%
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/mnist_6vs7_lsa_tlsa_mnist.png}
    %            \caption{mnist 6vs7}
    %            \label{fig:mnist_6vs7_lsa_tlsa_mnist}
    %    \end{subfigure}%
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/mnist_8vs9_lsa_tlsa_mnist.png}
                \caption{\textit{MNIST 8vs9}}
                \label{fig:mnist_8vs9_lsa_tlsa_mnist}
        \end{subfigure}%

\end{center}
\caption{Test Accuracy of LSA versus Transfer LSA on \textit{MNIST}}
\label{fig:lsa_tlsa_mnist}
\end{figure}


==> figure_tex/lsa_tlsa_usps.tex <==
\begin{figure}[t]
\begin{center}
\centering
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/usps_0vs1_lsa_tlsa_usps.png}
                \caption{\textit{USPS 0vs1}}
                \label{fig:usps_0vs1_lsa_tlsa_usps}
        \end{subfigure}%
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/usps_4vs5_lsa_tlsa_usps.png}
    %            \caption{usps 4vs5}
    %            \label{fig:usps_4vs5_lsa_tlsa_usps}
    %    \end{subfigure}%
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/usps_6vs7_lsa_tlsa_usps.png}
    %            \caption{usps 6vs7}
    %            \label{fig:usps_6vs7_lsa_tlsa_usps}
    %    \end{subfigure}%
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/usps_8vs9_lsa_tlsa_usps.png}
                \caption{\textit{USPS 8vs9}}
                \label{fig:usps_8vs9_lsa_tlsa_usps}
        \end{subfigure}%

\end{center}
\caption{Test Accuracy of LSA versus Transfer LSA on \textit{USPS}}
\label{fig:lsa_tlsa_usps}
\end{figure}


==> figure_tex/mnist_albl_talbl.tex <==
i


==> figure_tex/mnist_lsa_tlsa.tex <==
i


==> figure_tex/tlsa_talbl_mnist.tex <==
\begin{figure}[t]
\begin{center}
\centering
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/mnist_0vs1_tlsa_talbl_mnist}
                \caption{\textit{MNIST 0vs1}}
                \label{fig:mnist_0vs1_tlsa_talbl_mnist}
        \end{subfigure}%
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/mnist_2vs3_tlsa_talbl_mnist}
    %            \caption{mnist 2vs3}
    %            \label{fig:mnist_2vs3_tlsa_talbl_mnist}
    %    \end{subfigure}%
    %
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/mnist_6vs7_tlsa_talbl_mnist}
    %            \caption{mnist 4vs5}
    %            \label{fig:mnist_4vs5_tlsa_talbl_mnist}
    %    \end{subfigure}%
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/mnist_8vs9_tlsa_talbl_mnist}
                \caption{\textit{MNIST 8vs9}}
                \label{fig:gmnist_8vs9_tlsa_talbl_mnist}
        \end{subfigure}%

\end{center}
\caption{Test Accuracy of Transfer LSA versus other competitors on \textit{MNIST}}
\label{fig:tlsa_talbl_mnist}
\end{figure}


==> figure_tex/tlsa_talbl_usps.tex <==
\begin{figure}[t]
\begin{center}
\centering
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/usps_0vs1_tlsa_talbl_usps}
                \caption{\textit{USPS 0vs1}}
                \label{fig:usps_0vs1_tlsa_talbl_usps}
        \end{subfigure}%
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/usps_4vs5_tlsa_talbl_usps}
    %            \caption{usps 4vs5}
    %            \label{fig:usps_4vs5_tlsa_talbl_usps}
    %    \end{subfigure}%
    %
    %\begin{subfigure}[b]{0.25\textwidth}
    %            \includegraphics[width=\textwidth]{./matlab_figure/usps_6vs7_tlsa_talbl_usps}
    %            \caption{usps 6vs7}
    %            \label{fig:usps_6vs7_tlsa_talbl_usps}
    %    \end{subfigure}%
    \begin{subfigure}[b]{0.25\textwidth}
                \includegraphics[width=\textwidth]{./matlab_figure/usps_8vs9_tlsa_talbl_usps}
                \caption{\textit{USPS 8vs9}}
                \label{fig:gusps_8vs9_tlsa_talbl_usps}
        \end{subfigure}%

\end{center}
\caption{Test Accuracy of Transfer LSA versus other competitors on \textit{USPS}}
\label{fig:tlsa_talbl_usps}
\end{figure}

